What Makes a Place? Building Bespoke Place Dependent Object Detectors for Robotics

This paper is about enabling robots to improve their perceptual performance through repeated use in their operating environment, creating local expert detectors fitted to the places through which a robot moves. We leverage the concept of 'experiences' in visual perception for robotics, accounting for bias in the data a robot sees by fitting object detector models to a particular place. The key question we seek to answer in this paper is simply: how do we define a place? We build bespoke pedestrian detector models for autonomous driving, highlighting the necessary trade off between generalisation and model capacity as we vary the extent of the place we fit to. We demonstrate a sizeable performance gain over a current state-of-the-art detector when using computationally lightweight bespoke place-fitted detector models.

==> 06_deep_learning.tex <==
%!TEX root=main.tex

\section{Place Fitting and Deep Learning}
\label{sec:discussion-dl}

In comparing the results in Sections \ref{sec:ideal-place-spatial}-\ref{sec:ideal-place-similarity}, it is clear that one of the key factors for place-fitted detector performance is model capacity. If we try to fit a model to too large a negative class (to the point that we must make our model generalise) we see the performance degrade.

Recently, deep learning approaches to detection have been very successful on the various object detection benchmark datasets, and they are now approaching the run-time performance of classical detection methods. However, they frequently do not transfer well to other domains, meaning that these do not achieve the same level of performance on our urban driving data as the KITTI or Caltech urban driving benchmarks. 

Nevertheless, neural network object detectors do have significant representational capacity, and this offers potential gains in fitting models to a broader definition of a `place'. From the deep learning literature, we note parallels with `fine-tuning' a model to suit the class of data \cite{bengio2012practical,bengio2012deep}. Intuitively we can see why from Figure \ref{fig:caltech-v-oxford}: the training environment is drawn from driving in an urban environment, but it is quite different to the urban driving environment our robot operates in.

\begin{figure} [htbp]
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/deep-learning/set07_V001_I00749.jpg}
        \caption{Caltech (Los Angeles).}
        \label{fig:caltech-example}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{images/deep-learning/nthoxfjan.png}
    \caption{North Oxford.}
    \label{fig:nthoxfjan-example}
    \end{subfigure}
\caption{The data drawn from the Caltech dataset are visually distinct from our robot's operating environment.}
\label{fig:caltech-v-oxford}
\end{figure}


We evaluate the capacity of MSCNN \cite{cai2016unified} to fit one of our test routes. We partition our two labelled laps from the North Oxford January dataset (Table \ref{tab:test-imgs}), using the first lap as training data, and the second as test data. This is equivalent to  fitting a model to the full-lap test case in Section \ref{sec:ideal-place-spatial}, Figure \ref{fig:ideal-place-spatial-pr-mrfppi}.

We fit the model using the method in the second phase of training (fine-tuning) in \cite{cai2016unified}, but with the learning rate reduced by a factor of ten and the network weights initialised to the pretrained Caltech model supplied by the authors. 

After fitting the network to this route we see the detector performance jump thirty percentage points from moderate performance at 0.637 AP to a near-perfect 0.944 AP (Figure \ref{fig:mscnn-results}), an even greater improvement than place-fitting with classical models.  We see similar gains in all other metrics (Table \ref{tab:mscnn-performance}). The greater representational power of the MSCNN network allows it to successfully fit the environment along the entire route.


\begin{table}[htbp]
	\centering
    \begin{tabular}{| P{2.8cm} | P{1.1cm} | P{1.5cm} | P{0.9cm} |}
		\hline
		MSCNN Model & Average Precision & Log Average Miss Rate & Max F1 Score \\ 
		\hline
		Baseline (Caltech only) & 0.637 & 0.338 & 0.621 \\
		Place Fitted (N.Oxf.Jan) & \textbf{0.944} & \textbf{0.042} & \textbf{0.935} \\
		\hline
	\end{tabular}
	\caption{Performance metrics on the test lap of the North Oxford January Dataset.}
	\label{tab:mscnn-performance}
\end{table}

\begin{figure} [htbp]
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/deep-learning/nthoxfjan_finetuning_pr.eps}
        \caption{Average Precision (higher is better).}
        \label{fig:cent-oxf-avg-prec}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
    \centering
    	\includegraphics[width=\columnwidth]{images/deep-learning/nthoxfjan_finetuning_mrfppi.eps}
    	\caption{Log-Average Miss Rate (lower is better).}
    	\label{fig:cent-oxf-logavg-mr}
    \end{subfigure}
\caption{Performance metrics for two MSCNN models on the test lap of North Oxford January. The baseline model is supplied by the authors and trained on Caltech. When we fit the model to our robot's operating route we see a substantial gain in performance.}
\label{fig:mscnn-results}
\end{figure}
